UnlearnCanvas: Stylized Image Dataset for Enhanced Machine Unlearning Evaluation in Diffusion Models

The technological advancements in diffusion models (DMs) have demonstrated unprecedented capabilities in text-to-image generation and are widely used in diverse applications. However, they have also raised significant societal concerns, such as the generation of harmful content and copyright disputes. Machine unlearning (MU) has emerged as a promising solution, capable of removing undesired generative capabilities from DMs. However, existing MU evaluation systems present several key challenges that can result in incomplete and inaccurate assessments. To address these issues, we propose UnlearnCanvas, a comprehensive high-resolution stylized image dataset that facilitates the evaluation of the unlearning of artistic styles and associated objects. This dataset enables the establishment of a standardized, automated evaluation framework with 7 quantitative metrics assessing various aspects of the unlearning performance for DMs. Through extensive experiments, we benchmark 9 state-of-the-art MU methods for DMs, revealing novel insights into their strengths, weaknesses, and underlying mechanisms. Additionally, we explore challenging unlearning scenarios for DMs to evaluate worst-case performance against adversarial prompts, the unlearning of finer-scale concepts, and sequential unlearning. We hope that this study can pave the way for developing more effective, accurate, and robust DM unlearning methods, ensuring safer and more ethical applications of DMs in the future. The dataset, benchmark, and codes are publicly available at https://unlearn-canvas.netlify.app/.

==> sections/related_work.tex <==
\newpage
\section{Related Work}
\label{sec: related_work}

\paragraph{Machine Unlearning for Diffusion Models}
Machine unlearning, an emerging area within the field of machine learning, primarily aims at removing or reducing of the influence of specific data subsets {\cite{cao2015towards,golatkar2020eternal,warnecke2021machine,graves2021amnesiac,thudi2021unrolling,becker2022evaluating,izzo2021approximate}}. Initially conceived as a privacy safeguard {\cite{dwork2006our}}, its scope has since expanded to encompass other domains, including defense against backdoor attacks {\cite{liu2022backdoor}}, transfer learning {\cite{jia2023model}}, and more {\cite{koh2017understanding,warnecke2021machine, wang2022federated, wu2022federated,chien2022certified, cheng2023gnndelete}}.
Concurrently, the proliferation of large-scale text-conditioned diffusion-based generative models like StableDiffusion {\cite{rombach2022high}} and Imagen {\cite{saharia2022photorealistic}} has drawn increased attention to issues related to copyright and inappropriate content generation, prompting efforts to develop unlearning methods {\cite{gandikota2023erasing,zhang2023forget,kumari2023ablating,gandikota2023unified,schramowski2023safe}} to mitigate these concerns.
Early endeavors in this realm involved post-image filtering {\cite{schuhmann2022laion,rando2022red}} and modifications to inference guidance, resembling post-hoc interventions that did not fully address the underlying tendencies of models to generate undesirable content. Recent advancements have shifted toward retraining with curated datasets {\cite{rombach2022high}} and more practical fine-tuning techniques {\cite{gandikota2023erasing,zhang2023forget,kumari2023ablating,gandikota2023unified}}. 
% Style unlearning has played a pivotal role in many of these practical studies, focusing on disabling the model's ability to generate specific styles of images {\tocite}. 
{The concept of style unlearning has assumed a critical role in numerous empirical studies, and these investigations primarily concentrate on attenuating the model's capacity to produce images in particular styles.}
This mirrors the challenges posed by copyright concerns in generative models and has become a valuable testbed for contemporary generative machine unlearning methods. 
%{\tocite}. 
{Although various studies \cite{zhang2023generate, chin2023prompting4debugging} have been proposed to assess the efficacy of unlearning in generative models, focusing on diverse unlearning types such as object and concept unlearning from an attacker's perspective, our comprehensive evaluation specifically concentrates on style unlearning.}


\paragraph{Neural Style Transfer}
Style transfer aims to transfer the artistic style from one reference image (also termed as ``\textbf{s}tyle image'') $\bx_s$ to a \textbf{c}ontent image $\bx_c$, which is a long-standing topic and can be traced back to the time before deep neural networks were applied {\cite{hertzmann1998painterly,hertzmann2023image,wang2004efficient}}.
{\cite{gatys2015texture,gatys2015neural}} introduced the concept of Gram loss on deep neural features to represent image styles, marking the beginning of the neural style transfer era. This pioneering work inspired a series of subsequent studies, which can be broadly categorized into three classes based on their generalization abilities: the one-style-per-model approach {\cite{li2016combining,ulyanov2016instance,johnson2016perceptual,ulyanov2016texture,ulyanov2017improved,wang2017multimodal,risser2017stable,li2017laplacian}}, the multi-style-per-model approach {\cite{dumoulin2016learned,chen2017stylebank,gong2018neural}}, and the universal-style-transfer approach {\cite{li2017universal,huang2017arbitrary,chen2016fast,gu2018arbitrary,sheng2018avatar,an2020ultrafast,wang2020collaborative,lu2019closed,wang2020diversified,an2020real}}. The latter exhibits the highest level of generalization, making it applicable to unseen styles. Notably, \textsc{AdaIn} {\cite{huang2017arbitrary}} proposed adaptive instance normalization as a means to fuse content and style by aligning their statistical properties. Meanwhile, \textsc{WCT} {\cite{li2017universal}} devised a whitening and colorization transformation to match second-order statistics of content and style features. Several other methods have also introduced self-attention mechanisms within the encoder-transfer-decoder framework. \textsc{ArtFlow} {\cite{an2021artflow}} addressed content leakage issues in style transfer methods using reversible neural flows for lossless and unbiased image recovery. \textsc{IE-Contrast} {\cite{chen2021artistic}} introduced two types of contrastive loss to achieve harmonious and satisfactory stylization. More recently, \textsc{StyTr2} {\cite{deng2022stytr2}} utilized two transformer encoders, one for contents and one for styles, to capture domain-specific long-range information. 
%In contrast, \textsc{Cast} {\tocite} directly used image features by introducing a Multi-Scale Pooling (MSP) module for style encoding.
{Conversely, \textsc{Cast} {\cite{zhang2022domain}} employs image features directly through the introduction of a Multi-Scale Pooling (MSP) module, which is utilized for style encoding.}
With the emergence of diffusion models {\cite{saharia2022photorealistic, rombach2022high, ramesh2022hierarchical, nichol2021glide}}, some diffusion-based methods have also demonstrated the ability to extract style features from one or a series of style images and apply them to new content features. For instance, \textsc{Blip} introduced a multimodal encoder to capture subject representation, enabling zero-shot subject-driven generation, which includes style transfer as a special case. 
%Another line of work, referred to as learning-based neural style transfer {\tocite}, involves ``training'' or ``optimizing'' the inversion of a target style and before utilizing the learned features to perform style transfer. This approach differs from style transfer, as it typically requires a training process {\tocite}. 
Another line of research {\cite{chefer2022image,gal2022image}} involves the `training' or `optimizing' the inversion of a given target style, followed by the application of these learned features for executing the style transfer. 
% \SL{[why needs the following sentence?]}
% This methodology diverges fundamentally from conventional style transfer techniques, primarily due to its reliance on a comprehensive training process \tocite.
Some variants of these method can also utilize multiple style images to enhance the performance, and representative works include \textsc{StyleDrop} {\cite{sohn2023styledrop}}, \textsc{InST} {\cite{zhang2023inversion}}, and \textsc{Prospect} {\cite{zhang2023prospect}}.
